Invariance-inducing regularization using worst-case transformations suffices to boost accuracy and spatial robustness

This work provides theoretical and empirical evidence that invariance-inducing regularizers can increase predictive accuracy for worst-case spatial transformations (spatial robustness). Evaluated on these adversarially transformed examples, we demonstrate that adding regularization on top of standard or adversarial training reduces the relative error by 20% for CIFAR10 without increasing the computational cost. This outperforms handcrafted networks that were explicitly designed to be spatial-equivariant. Furthermore, we observe for SVHN, known to have inherent variance in orientation, that robust training also improves standard accuracy on the test set. We prove that this no-trade-off phenomenon holds for adversarial examples from transformation groups in the infinite data limit.

==> cifar_defenses_main.tex <==
\begin{table*}[ht]
\caption{Accuracies of different models trained with $\wok$ and first-order defenses and evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on the CIFAR-10 and CIFAR-100 datasets. Results on SVHN can be found in Table~\ref{tab:wok_svhn} in the Supplementary Materials, along with additional results for CIFAR-10 and CIFAR-100. \label{tab:wok_main}}
\vskip 0.15in
\begin{center}
{\renewcommand{\arraystretch}{1.4}
\begin{tabular}{cl|ccc|cc|cc}
& \diagbox{Training}{Evaluation} & Natural & Grid  \\

%% \hline
%% \multirow{10}{*}{\rotatebox[origin=c]{90}{SVHN}}
%% %%%%% Standard %%%%%%%%%%
%% & Standard
%%     & 95.48\% (0.15\%) & 18.85\% (1.27\%)\\
%% \cdashline{2-4}
%% %%%%% FO %%%%%%%%%%
%% & $\recovarit{\atabb}{\fo}{50}$ 
%% 	& 96.27\% (0.00\%) &  84.81\% (0.01\%)\\
%% & $\recovarit{\atabb}{\fo}{100}$ 
%% 	& 96.06\% (0.10\%) & 87.29\% (0.09\%)\\
%% & $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 2.5$)
%% 	& 96.30\% (0.09\%) & {\bf 92.42\% (0.20\%)}\\
%% \cdashline{2-4}
%% %%%%% Worst-of-1 %%%%%%%%%%	
%% &  $\recovarit{\atabb}{\woabb{1}}{50}$
%% 	& 96.19\% (0.06\%) & 80.43\% (0.14\%)\\
%% &  $\recovarit{\atabb}{\woabb{1}}{100}$
%% 	& 93.97\% (0.09\%) & 82.60\% (0.23\%)\\
%% & $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%% 	& 96.19\% (0.07\%) & {\bf 90.48\% (0.15\%)}\\ 
%% \cdashline{2-4}
%% %%%%% Worst-of-10 %%%%%%%%%%		
%% &  $\atabb$ with $\woabb{10}$ $\half$
%%     & {96.56\% (0.07\%)} & 88.83\% (0.10\%) \\
%% &  $\recovarit{\atabb}{\woabb{10}}{50}$
%%     & 95.92\% (0.03\%) & 89.75\% (0.17\%) \\
%% & $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1.5$)
%%     & 96.41\% (0.07\%) & {\bf 92.17\% (0.11\%)}  \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
%%%%%% Standard %%%%%%%%%%
%& Standard
%    & 92.11\% (0.18\%) & 9.52\% (0.66\%)  \\
%%& No Crop
%%    & 90.50\% (0.22\%) & 1.63\% (0.21\%)  \\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%
%&  $\recovarit{\atabb}{\woabb{1}}{50}$
%	& 92.96\% (0.17\%) & 51.27\% (0.45\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 89.93\% (0.18\%) & 58.29\% (0.60\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%	& 89.43\% (0.28\%) & {\bf 71.97\% (0.11\%)}\\
%	\cdashline{2-4}
%%%%% Worst-of-10 %%%%%%%%%%
&  $\recovarit{\atabb}{\woabb{10}}{50}$
    & {93.44\% (0.19\%)} & 68.14\% (0.48\%) \\
&  $\recovarit{\atabb}{\woabb{10}}{100}$
    & 92.05\% (0.25\%) & 70.35\% (0.17\%) \\
& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1$)
    & 91.13\% (0.13\%) & {\bf 75.89\% (0.23\%)}  \\
 \cdashline{2-4}
%%%%% FO %%%%%%%%%%
& $\recovarit{\atabb}{\fo}{50}$ 
	& 92.19\% (0.23\%) & 64.26\% (0.25\%)\\
& $\recovarit{\atabb}{\fo}{100}$ 
	& 91.83\% (0.19\%)& 69.74\% (0.27\%)\\
& $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 3$)
	& 89.70\% (0.10\%) & {\bf 77.72\% (0.35\%)}\\

\hline                                                                              
\multirow{6}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
%& Standard
%    & 70.23\% (0.18\%) & 5.09\% (0.25\%)  \\
%%& No Crop
%%    & 66.42\% (0.30\%) & 0.86\% (0.08\%)  \\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%	
%&  $\recovarit{\atabb}{\woabb{1}}{50}$
%	& 72.38\% (0.17\%) & 23.43\% (0.47\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 66.62\% (0.37\%) & 28.53\% (0.25\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 0.75$)
%	& 66.54\% (0.26\%) & {\bf 45.97\% (0.22\%)}\\
%	\cdashline{2-4}
%%%%% Worst-of-10 %%%%%%%%%%
&  $\recovarit{\atabb}{\woabb{10}}{50}$
    & {73.03\% (0.13\%)} & 35.93\% (0.24\%) \\
&  $\recovarit{\atabb}{\woabb{10}}{100}$
    & 68.79\% (0.34\%) & 38.21\% (0.10\%) \\
& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 0.25$)
    & 68.54\% (0.27\%) & {\bf 49.30\% (0.33\%)} \\
\cdashline{2-4}
%%%%% FO %%%%%%%%%%
& $\recovarit{\atabb}{\fo}{50}$ 
	& 71.11\% (0.37\%) & 33.40\% (0.21\%) \\
& $\recovarit{\atabb}{\fo}{100}$ 
	& 68.87\% (0.19\%) & 37.87\% (0.12\%) \\
&$\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 0.5$)
	&  68.44\% (0.39\%) & {\bf 52.58\% (0.20\%)} \\

\end{tabular}}
\end{center}
\end{table*}


==> cifar_defenses_main_narrow.tex <==
\begin{table}[h]
\caption{\small Mean accuracies of models trained with $\wokabb$ and $\fo$ defenses and evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on the CIFAR datasets. Results on SVHN can be found in Table~\ref{tab:wok_svhn}, additional results for CIFAR are contained in Table~\ref{tab:wok_cifar}. \label{tab:wok_main}}
%\vskip 0.15in
\begin{center}
{\renewcommand{\arraystretch}{1.4}
\begin{tabular}{cl|ccc|cc|cc}
& \diagbox{Training}{Evaluation} & Natural & Grid  \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
%%%%% Worst-of-10 %%%%%%%%%%
&  $\recovarit{\atabb}{\woabb{10}}{50}$
    & {93.44\%} & 68.14\% \\
&  $\recovarit{\atabb}{\woabb{10}}{100}$
    & 92.05\% & 70.35\% \\
& $\recovarit{\acronymmath}{\woabb{10}}{50}$ %($\lambda = 1$)
    & 91.13\% & {\bf 75.89\%}  \\
 \cdashline{2-4}
%%%%% FO %%%%%%%%%%
& $\recovarit{\atabb}{\fo}{50}$ 
	& 92.19\% & 64.26\% \\
& $\recovarit{\atabb}{\fo}{100}$ 
	& 91.83\% & 69.74\% \\
& $\recovarit{\acronymmath}{\fo}{50}$ %($\lambda = 3$)
	& 89.70\%  & {\bf 77.72\%}\\

\hline                                                                              
\multirow{6}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
%%%%% Worst-of-10 %%%%%%%%%%
&  $\recovarit{\atabb}{\woabb{10}}{50}$
    & {73.03\% } & 35.93\% \\
&  $\recovarit{\atabb}{\woabb{10}}{100}$
    & 68.79\%  & 38.21\% \\
& $\recovarit{\acronymmath}{\woabb{10}}{50}$ %($\lambda = 0.25$)
    & 68.54\% & {\bf 49.30\% } \\
\cdashline{2-4}
%%%%% FO %%%%%%%%%%
& $\recovarit{\atabb}{\fo}{50}$ 
	& 71.11\%  & 33.40\%  \\
& $\recovarit{\atabb}{\fo}{100}$ 
	& 68.87\%  & 37.87\%  \\
&$\recovarit{\acronymmath}{\fo}{50}$ %($\lambda = 0.5$)
	&  68.44\% & {\bf 52.58\%} \\
\end{tabular}}
\end{center}
\end{table}
%\vskip -0.05in

==> cifar_table.tex <==
%% \begin{table}[H]
%%     \caption{Mean accuracies of different models trained with and without regularizers and evaluated on the natural test set and against the grid search attack on CIFAR-100. Standard errors are shown in parentheses.}
%%     \label{tab:wok_cifar}
%%     \begin{center}
%%   \vskip 0.15in
%% 	%{\stdaug refers to data augmentation, i.e. \ltwo (\advb, \dataug, \rnd). Accuracies of different models trained with $\woabb{1}$ defenses (corresponding to data augmentation) and evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on the CIFAR-10 and CIFAR-100 datasets.
%%    {\setlength{\tabcolsep}{4pt}
%% 	 \begin{tabular}{c c c c c c}
%% 	 &\std & $\AT(\mix,\rnd)$& $\AT(\rob,\rnd) \equiv \aug{\std}$&	$\ALP(\mix,\rnd)$ ($\lambda = 0.75$) &\\
%%      \hline
%% 	CIFAR100 (nat) &70.23 (0.18)& 72.38 (0.17)&	66.62 (0.37)&	66.54 (0.26) & \\
%% 	\qquad\quad\quad (grid) &5.09 (0.25)&  23.43 (0.47)&	28.53 (0.25)&	{\bf 45.97 (0.22)}&\\
%%     \hdashline
%%      && $\AT(\mix,\woabb{10})$& $\AT(\rob,\woabb{10})$&	$\ALP(\mix,\woabb{10})$ ($\lambda = 0.25$) &\\
%%      \hline
%%      CIFAR100 (nat) && 73.03 (0.13)&	68.79 (0.34)&	68.54 (0.27) & \\
%%      \qquad\quad\quad (grid) &&  35.93 (0.24)&	38.21 (0.10)&	{\bf 49.30 (0.33)}&\\
%%      \hdashline
%%      && $\AT(\mix,\woabb{20})$& $\AT(\rob,\woabb{20})$&	$\ALP(\mix,\woabb{20})$ ($\lambda = 0.25$) &\\
%%      \hline
%%      CIFAR100 (nat) && 73.33 (0.22)&	69.15 (0.49)&	68.04 (0.27) & \\
%%      \qquad\quad\quad (grid) &&  38.06 (0.19)&	40.09 (0.31)&	{\bf 49.98 (0.31)}&\\
%%      \hdashline
%%      && $\AT(\mix,\fo)$& $\AT(\rob,\fo)$&	$\ALP(\mix,\fo)$ ($\lambda = 0.5$) &\\
%%     \hline
%%     CIFAR100 (nat) && 71.11 (0.37)&	68.87 (0.19)&	68.44 (0.39) & \\
%%     \qquad\quad\quad (grid) &&  33.40 (0.21)&	37.87 (0.12)&	{\bf 52.58 (0.20)}&\\

   
%%     \end{tabular}}
%% \end{center}
%% \end{table}






% \begin{table*}[htp]
%   \caption{Mean accuracies of different models trained with and without regularizers and evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on CIFAR-100. Standard errors are shown in parentheses.}
%     \label{tab:wok_cifar}
% \vskip 0.15in

% \begin{center}
% {\renewcommand{\arraystretch}{1.4}
% \begin{tabular}{cl|ccc|cc|cc}
% & \diagbox{Training}{Evaluation} & Natural & Grid  \\
% \hline
%\multirow{13}{*}{\rotatebox[origin=c]{90}{SVHN}}
%%%%%%% Standard %%%%%%%%%%
%& Standard
%    & 95.48\% (0.15\%) & 18.85\% (1.27\%)\\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%	
%&  $\AT(\mix,{\woabb{1}})$
%	& 96.19\% (0.06\%) & 80.43\% (0.14\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 93.97\% (0.09\%) & 82.60\% (0.23\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%	& 96.19\% (0.07\%) & {\bf 90.48\% (0.15\%)}\\ 
%\cdashline{2-4}
%%%%%% Worst-of-10 %%%%%%%%%%		
%&  $\recovarit{\atabb}{\woabb{10}}{50}$
%    & {96.56\% (0.07\%)} & 88.83\% (0.10\%) \\
%&  $\recovarit{\atabb}{\woabb{10}}{100}$
%    & 95.92\% (0.03\%) & 89.75\% (0.17\%) \\
%& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1.5$)
%    & 96.41\% (0.07\%) & {\bf 92.17\% (0.11\%)}  \\
%\cdashline{2-4}
%%%%%% Worst-of-20 %%%%%%%%%%		
%&  $\recovarit{\atabb}{\woabb{20}}{50}$
%    & 96.60\% (0.06\%) & 89.72\% (0.17\%) \\
%&  $\recovarit{\atabb}{\woabb{20}}{100}$
%    & 96.29\% (0.14\%) & 90.57\% (0.20\%) \\
%& $\recovarit{\acronymmath}{\woabb{20}}{50}$ ($\lambda = 1.5$)
%    & 96.39\% (0.04\%) & {\bf 92.48\% (0.05\%)} \\
%\cdashline{2-4}
%%%%%% FO %%%%%%%%%%
%& $\recovarit{\atabb}{\fo}{50}$ 
%	& 96.27\% (0.00\%) &  84.81\% (0.01\%)\\
%& $\recovarit{\atabb}{\fo}{100}$ 
%	& 96.06\% (0.10\%) & 87.29\% (0.09\%)\\
%& $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 2.5$)
%	& 96.30\% (0.09\%) & {\bf 92.42\% (0.20\%)}\\    
%\hline
%\multirow{13}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
%%%%%% Standard %%%%%%%%%%
%& Standard
%    & 92.11\% (0.18\%) & 9.52\% (0.66\%)  \\
%%& No Crop
%%    & 90.50\% (0.22\%) & 1.63\% (0.21\%)  \\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%
%&  $\AT(\mix,{\woabb{1}})$
%	& 92.96\% (0.17\%) & 51.27\% (0.45\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 89.93\% (0.18\%) & 58.29\% (0.60\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%	& 89.43\% (0.28\%) & {\bf 71.97\% (0.11\%)}\\
%\cdashline{2-4}
%%%%%% Worst-of-10 %%%%%%%%%%
%&  $\recovarit{\atabb}{\woabb{10}}{50}$
%    & {93.44\% (0.19\%)} & 68.14\% (0.48\%) \\
%&  $\recovarit{\atabb}{\woabb{10}}{100}$
%    & 92.05\% (0.25\%) & 70.35\% (0.17\%) \\
%& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1$)
%    & 91.13\% (0.13\%) & {\bf 75.89\% (0.23\%)}  \\
% \cdashline{2-4}
%%%%%% Worst-of-20 %%%%%%%%%%		
%&  $\recovarit{\atabb}{\woabb{20}}{50}$
%    & 93.46\% (0.17\%) & 69.98\% (0.22\%) \\
%&  $\recovarit{\atabb}{\woabb{20}}{100}$
%    & 92.15\% (0.28\%) & 72.31\% (0.20\%) \\
%& $\recovarit{\acronymmath}{\woabb{20}}{50}$ ($\lambda = 1$)
%    & 90.67\% (0.12\%) & {\bf 76.72\% (0.21\%)} \\
%    \cdashline{2-4}
%%%%%% FO %%%%%%%%%%
%& $\recovarit{\atabb}{\fo}{50}$ 
%	& 92.19\% (0.23\%) & 64.26\% (0.25\%)\\
%& $\recovarit{\atabb}{\fo}{100}$ 
%	& 91.83\% (0.19\%)& 69.74\% (0.27\%)\\
%& $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 3$)
%	& 89.70\% (0.10\%) & {\bf 77.72\% (0.35\%)}\\
%\hline                                                                              
% \multirow{13}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
% %%%%% Standard %%%%%%%%%%
% & std
%     & 70.23\% (0.18\%) & 5.09\% (0.25\%)  \\
% %& No Crop
% %    & 66.42\% (0.30\%) & 0.86\% (0.08\%)  \\
% \cdashline{2-4}
% %%%%% Worst-of-1 %%%%%%%%%%	
% &  $\AT(\mix,{\rnd})$
% 	& 72.38\% (0.17\%) & 23.43\% (0.47\%)\\
% &  $\AT(\rob,{\rnd}) \equiv \aug{\std}$
% 	& 66.62\% (0.37\%) & 28.53\% (0.25\%)\\
% & $\ALP(\mix,\rnd)$ ($\lambda = 0.75$)
% 	& 66.54\% (0.26\%) & {\bf 45.97\% (0.22\%)}\\
% 	\cdashline{2-4}
% %%%%% Worst-of-10 %%%%%%%%%%
% &  $\AT(\mix,{\woabb{10}})$
%     & {73.03\% (0.13\%)} & 35.93\% (0.24\%) \\
% &  $\AT(\rob,{\woabb{10}})$
%     & 68.79\% (0.34\%) & 38.21\% (0.10\%) \\
% & $\ALP(\mix,\woabb{10})$ ($\lambda = 0.25$)
%     & 68.54\% (0.27\%) & {\bf 49.30\% (0.33\%)} \\
% \cdashline{2-4}

% %%%%% Worst-of-20 %%%%%%%%%%		
% &  $\AT(\mix,{\woabb{20}})$
%     & 73.33\% (0.22\%) & 38.06\% (0.19\%) \\
% &  $\AT(\rob,{\woabb{20}})$
%     & 69.15\% (0.49\%) & 40.09\% (0.31\%) \\
% & $\ALP(\mix,\woabb{20})$ ($\lambda = 0.25$)
%     & 68.04\% (0.27\%) & {\bf 49.98\% (0.31\%)} \\
%     \cdashline{2-4}
% %%%%% FO %%%%%%%%%%
% & $\AT(\mix,{\fo})$ 
% 	& 71.11\% (0.37\%) & 33.40\% (0.21\%) \\
% & $\AT(\rob,{\fo})$ 
% 	& 68.87\% (0.19\%) & 37.87\% (0.12\%) \\
% &$\ALP(\mix,{\fo})$ ($\lambda = 0.5$)
% 	&  68.44\% (0.39\%) & {\bf 52.58\% (0.20\%)} \\
% \end{tabular}}
% \end{center}
% \end{table*}




%\begin{table*}[htp]
%  \caption{Mean accuracies of different models trained with and without defenses and evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on the CIFAR-10 and CIFAR-100 datasets. Standard errors are shown in parentheses.}
%    \label{tab:wok_cifar}
%\vskip 0.15in
%
%\begin{center}
%{\renewcommand{\arraystretch}{1.4}
%\begin{tabular}{cl|ccc|cc|cc}
%& \diagbox{Training}{Evaluation} & Natural & Grid  \\
%\hline
%%\multirow{13}{*}{\rotatebox[origin=c]{90}{SVHN}}
%%%%%%%% Standard %%%%%%%%%%
%%& Standard
%%    & 95.48\% (0.15\%) & 18.85\% (1.27\%)\\
%%\cdashline{2-4}
%%%%%%% Worst-of-1 %%%%%%%%%%	
%%&  $\AT(\mix,{\woabb{1}})$
%%	& 96.19\% (0.06\%) & 80.43\% (0.14\%)\\
%%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%%	& 93.97\% (0.09\%) & 82.60\% (0.23\%)\\
%%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%%	& 96.19\% (0.07\%) & {\bf 90.48\% (0.15\%)}\\ 
%%\cdashline{2-4}
%%%%%%% Worst-of-10 %%%%%%%%%%		
%%&  $\recovarit{\atabb}{\woabb{10}}{50}$
%%    & {96.56\% (0.07\%)} & 88.83\% (0.10\%) \\
%%&  $\recovarit{\atabb}{\woabb{10}}{100}$
%%    & 95.92\% (0.03\%) & 89.75\% (0.17\%) \\
%%& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1.5$)
%%    & 96.41\% (0.07\%) & {\bf 92.17\% (0.11\%)}  \\
%%\cdashline{2-4}
%%%%%%% Worst-of-20 %%%%%%%%%%		
%%&  $\recovarit{\atabb}{\woabb{20}}{50}$
%%    & 96.60\% (0.06\%) & 89.72\% (0.17\%) \\
%%&  $\recovarit{\atabb}{\woabb{20}}{100}$
%%    & 96.29\% (0.14\%) & 90.57\% (0.20\%) \\
%%& $\recovarit{\acronymmath}{\woabb{20}}{50}$ ($\lambda = 1.5$)
%%    & 96.39\% (0.04\%) & {\bf 92.48\% (0.05\%)} \\
%%\cdashline{2-4}
%%%%%%% FO %%%%%%%%%%
%%& $\recovarit{\atabb}{\fo}{50}$ 
%%	& 96.27\% (0.00\%) &  84.81\% (0.01\%)\\
%%& $\recovarit{\atabb}{\fo}{100}$ 
%%	& 96.06\% (0.10\%) & 87.29\% (0.09\%)\\
%%& $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 2.5$)
%%	& 96.30\% (0.09\%) & {\bf 92.42\% (0.20\%)}\\    
%%\hline
%\multirow{13}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
%%%%%% Standard %%%%%%%%%%
%& Standard
%    & 92.11\% (0.18\%) & 9.52\% (0.66\%)  \\
%%& No Crop
%%    & 90.50\% (0.22\%) & 1.63\% (0.21\%)  \\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%
%&  $\AT(\mix,{\woabb{1}})$
%	& 92.96\% (0.17\%) & 51.27\% (0.45\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 89.93\% (0.18\%) & 58.29\% (0.60\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%	& 89.43\% (0.28\%) & {\bf 71.97\% (0.11\%)}\\
%\cdashline{2-4}
%%%%%% Worst-of-10 %%%%%%%%%%
%&  $\recovarit{\atabb}{\woabb{10}}{50}$
%    & {93.44\% (0.19\%)} & 68.14\% (0.48\%) \\
%&  $\recovarit{\atabb}{\woabb{10}}{100}$
%    & 92.05\% (0.25\%) & 70.35\% (0.17\%) \\
%& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1$)
%    & 91.13\% (0.13\%) & {\bf 75.89\% (0.23\%)}  \\
% \cdashline{2-4}
%%%%%% Worst-of-20 %%%%%%%%%%		
%&  $\recovarit{\atabb}{\woabb{20}}{50}$
%    & 93.46\% (0.17\%) & 69.98\% (0.22\%) \\
%&  $\recovarit{\atabb}{\woabb{20}}{100}$
%    & 92.15\% (0.28\%) & 72.31\% (0.20\%) \\
%& $\recovarit{\acronymmath}{\woabb{20}}{50}$ ($\lambda = 1$)
%    & 90.67\% (0.12\%) & {\bf 76.72\% (0.21\%)} \\
%    \cdashline{2-4}
%%%%%% FO %%%%%%%%%%
%& $\recovarit{\atabb}{\fo}{50}$ 
%	& 92.19\% (0.23\%) & 64.26\% (0.25\%)\\
%& $\recovarit{\atabb}{\fo}{100}$ 
%	& 91.83\% (0.19\%)& 69.74\% (0.27\%)\\
%& $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 3$)
%	& 89.70\% (0.10\%) & {\bf 77.72\% (0.35\%)}\\
%\hline                                                                              
%\multirow{13}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
%%%%%% Standard %%%%%%%%%%
%& Standard
%    & 70.23\% (0.18\%) & 5.09\% (0.25\%)  \\
%%& No Crop
%%    & 66.42\% (0.30\%) & 0.86\% (0.08\%)  \\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%	
%&  $\AT(\mix,{\woabb{1}})$
%	& 72.38\% (0.17\%) & 23.43\% (0.47\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 66.62\% (0.37\%) & 28.53\% (0.25\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 0.75$)
%	& 66.54\% (0.26\%) & {\bf 45.97\% (0.22\%)}\\
%	\cdashline{2-4}
%%%%%% Worst-of-10 %%%%%%%%%%
%&  $\recovarit{\atabb}{\woabb{10}}{50}$
%    & {73.03\% (0.13\%)} & 35.93\% (0.24\%) \\
%&  $\recovarit{\atabb}{\woabb{10}}{100}$
%    & 68.79\% (0.34\%) & 38.21\% (0.10\%) \\
%& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 0.25$)
%    & 68.54\% (0.27\%) & {\bf 49.30\% (0.33\%)} \\
%\cdashline{2-4}
%
%%%%%% Worst-of-20 %%%%%%%%%%		
%&  $\recovarit{\atabb}{\woabb{20}}{50}$
%    & 73.33\% (0.22\%) & 38.06\% (0.19\%) \\
%&  $\recovarit{\atabb}{\woabb{20}}{100}$
%    & 69.15\% (0.49\%) & 40.09\% (0.31\%) \\
%& $\recovarit{\acronymmath}{\woabb{20}}{50}$ ($\lambda = 0.25$)
%    & 68.04\% (0.27\%) & {\bf 49.98\% (0.31\%)} \\
%    \cdashline{2-4}
%%%%%% FO %%%%%%%%%%
%& $\recovarit{\atabb}{\fo}{50}$ 
%	& 71.11\% (0.37\%) & 33.40\% (0.21\%) \\
%& $\recovarit{\atabb}{\fo}{100}$ 
%	& 68.87\% (0.19\%) & 37.87\% (0.12\%) \\
%&$\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 0.5$)
%	&  68.44\% (0.39\%) & {\bf 52.58\% (0.20\%)} \\
%\end{tabular}}
%\end{center}
%\end{table*}
%


==> main_nips.tex <==
\section{Regularized for adversarially robust training (REGART)}
In this section we introduce a rigorous and unified framework for regularized
training for adversarial robustness. This framework includes theoretical justification for
many commonly used methods in adversarial training (mixed vs. all adv. batch, TRADES, ALP)
and includes new ones.

We then use these regularized estimators and compare with networks which are designed
to be ...

%% adds context to ALP/how we should reason about
%% ALP/reasons ALP might fail.  \fycomment{Along these lines: motivate
%%   the model and notation a bit more}

%% We then define the adversarial setting and introduce our general
%% framework for regularized adversarial training.  It then naturally
%% follows from the probabilistic model that the proposed penalized
%% regularization method leads to a robust classifier for an infinite regularization weight \fycomment{$\infty$ really...?}\chcomment{changed that.. }, stated more
%% formally in Theorem~\ref{prop}. This serves as a theoretical
%% justification to use \acronym and hence ALP.
Although our framework can
be applied broadly, we focus on image
classification as the prediction task of interest.


In adversarial robustness, you want robustness against changes against
transformations in your input which do not change the nature of your input.
This allows the
practitioner to know that even the most adversarial perturbation
$\Pert$ would not have influenced the probability of correct classification.
In the next section we introduce mathematical notation to think about this.


\subsection{Setting up transformation sets}
\label{sec:core}

The classifier $\func$ lies in a function space
$\param \in \RN^{\dimparam}$ and we denote the sample-wise loss
function on an observed pair $(X,Y)$ as $ \loss(\func_\param(X), Y)$
with examples being the 0-1 or cross entropy loss for classification.
We denote transformations of $X$ as $\Trafo{X}{\Pert}$ parameterized
by a perturbation vector $\Pert \in \Pertset \subset \RN^\dimpert$
such that the set of all possible transformations forms a
transformation group $\Group$ (i.e. closed).
We assume that our observations $X \in \RN^d$, $\ID \in \mathbb{Z}$, \Christina{need to introduce}
class $Y \in \RN$ are random variables drawn from a joint distribution
$\P$ over $(\ID, X,Y)$

We have a group $\Group$ of transformations $\Trafo{\cdot}{\Pert}$
of $\X$ onto itself. 
We denote by $\Gorbit{z}$ the $\Group$-orbit of $z$, that is
\begin{equation*}
\Gorbit{z} \defn \{ \Trafo{z}{\Pert}: \Trafo{\cdot}{\Pert} \in \Group\}.
\end{equation*}
\Christina{i.e. in words .. }
Note that for all $x, x'\in\Gorbit{z}$ we have $\Gorbit{x} =
\Gorbit{x'}$ by definition.  The random variable $X \in \Gorbit{z}$
for some $z$. Note that for $x' \not \in \Gorbit{z}$ we have
$\Gorbit{x} \cap \Gorbit{x'} = \emptyset$.  Therefore, for every $x$
there exists a unique $\Gorbit{z}$ such that $x\in \Gorbit{z}$. Thus
we abuse notation a little bit denote by $\Gorbit{X}$ the orbit
$\Gorbit{z}$ for which $X \in\Gorbit{z}$.  \Christina{At polishing stage: remove ``note that'' 's :-)} \Christina{Here: go through example where transformation is rotation only and describe what the notation corresponds to; below: pick up same example to illustrate $\SubGorbit{z}$; alternatively, consider moving generative model + DAG further up to illustrate ideas? }

\paragraph{Technicality for bounded subsets}
For our problem setting, transformations that form a closed group constitute too large a
set as adversarial attacks are
typically judged against the standard whether 
humans would misjudge an image. If the transformation is too large,
this restriction is not fulfilled anymore. \fycomment{hmm think...}
Mathematically this is similar to assuming a distribution on
$\Gorbit{z}$ for every $z$. It could have finite support. \Christina{connect this better to what follows or remove}

Hence, instead of transformation groups with $\Group$-orbits, we
consider connected subsets of orbits $\SubGorbit{z} \subset \Gorbit{z}$.  We
assume that these correspond to a set of ``maximal'' transformations $\Pertset_z$
defined by the diameter
\begin{equation}
  \label{eq:pertdiam}
  \Pertdiam_z = \max_{x',x\in\SubGorbit{z}} \|\Pert\|_2 \:\:\text{s.t. } x' = \Trafo{x}{\Pert}
\end{equation}
and $\Pertset_z = (-\Pertdiam_z, \Pertdiam_z)$ \fycomment{Notation not
  rigorous for the general transformation case...}  We assume that
$\Pertdiam$ is constant for all orbits and hence omit the $z$. For
example for rotations it makes sense that the feasible rotation range
for an image to not confuse a human to be the same for each image.
\fycomment{add how l-p balls fit here} Note that furthermore,
$\SubGorbit{z}$ do not overlap \fycomment{assume that or they don't}
and hence can still define the random variable $\SubGorbit{X} =
\SubGorbit{z}$ for $X \in \SubGorbit{z}$.

\subsection{Theoretical justification for regularization on the natural loss}


In adversarial robustness, the goal is for each $z$ to achieve the
same 0-1 loss for all observable images $X \in \SubGorbit{z}$.
The following loss function, common in the robust optimization
literature~\cite{BenTal09}, captures this adversarial
  concept
\begin{equation}
  \label{eq:advmin}
  \min_{f\in\Fspace} \EE_{X,Y} \sup_{x' \in\SubGorbit{X}} \loss(f(x'), Y)
\end{equation}
\fycomment{note about 0-1 loss vs. others (TRADES fuzz)}

%% \paragraph{Story overview}
%% \begin{itemize}
%% \item Theorem 1: for all $\epsilon$ we have that any robust solution (to the population problem) has to satisfy $f\in \InvF$. 
%% \item As a consequence, several $R(f) = 0$, and thus we can add that to $sup$ thing (with a problem *). Could also add to natural if it actually worked
%% \item Theorem 2: Natural s.t. $R(f) = 0$ yields robust solution
%% \item In reality we don't enforce $=0$ (with large lambda) because we have problems in optimization getting stuck in local optima
%% \item *Problem here is that we theoretically have to do two adversarial searches (one for $L$ and one for regularizer) - could handwave/argue that using adversarial examples of $L$ is a good approximation? \fycomment{somehow changing the example made a big difference for TRADES}
%% \item Could add that for linear case we can also directly say something about generalizability of robustness for linear transformations.
%% \item natural vs. robust accuracy: Under assumption~\eqref{eq:robustsense} there is no tradeoff.
%% \end{itemize}

%% Another way (more like it's now)
%% \begin{itemize}
%% \item Like in TRADES, can write the triangle like inequality, then use Lipschitz etc. - not so sure how to get TRADES ... 
%% \item Run all experiments with natural batch.
%% \item Theorem 1 & 2. 
%% \end{itemize}

 
%% Adversarial loss minimization
%% \begin{equation}
%%   \label{eq:advmin}
%%   \frob = \argmin_{f\in\Fspace} \EE_{X,Y} \sup_{x' \in\SubGorbit{X}} \loss(f(x'), Y)
%% \end{equation}

Let us denote as $\InvF$ the space of functions
which are constant on every $\SubGorbit{x}$ and define
a more general constraint
\begin{equation*}
  \InvF(\Reg) := \{f \in\Fspace: \Reg(f) = 0\} 
\end{equation*}
where we denote $\InvF := \InvF(\Reg_0)$ with $\Reg_0(f) = \sup_{x'\in
  \SubGorbit{x}} \|f(x) - f(x')\|_2$. For this and next section the reader
should think of $\Reg=\Reg_0$. A longer list of concrete regularizers that map
previous work to this framework is listed in Section~\ref{sec:diffreg}

\begin{theo}
  \label{theo:1}
    If $\InvF \subset \Fspace$, for every minimizer of adversarial loss~\eqref{eq:advmin} we have $\frob \in \InvF$.
\end{theo}

\begin{proof}
  Proof by contradiction. Let us assume that $\frob \not \in \InvF$. Let's denote the different values in the set $A = \{ \frob(x): x\in \SubGorbit{x} \}$. Denote the distribution over $x\in\SubGorbit{x}$ by $P_x$ we can rewrite the robust loss.
  \begin{align}
    \label{eq:prooflem}
    \min_{f\in\Fspace} \EE_{X,Y} \sup_{x' \in\SubGorbit{X}} \loss(f(x'), Y) = \EE_X [\EE_{Y|X} \sup_{x' \in \SubGorbit{X}} \loss(f(x'), Y)|\SubGorbit{x}] &\geq \int \sup_{a\in A} H(x, a) d P_x
  \end{align}
  where the function $H$ is specific to $\SubGorbit{x}$ and defined as $H(x,a) = \EE_{Y|x}\loss(a,Y)$. The right hand side is minimized by choosing $A = \{\abest\}$ with $\abest = \argmin_a \int H(x,a)d P_x$. Since setting $f(x) = \abest$ for all $x\in \SubGorbit{x}$ leads to equality in equation~\eqref{eq:prooflem}, q.e.d.
\end{proof}

Constrained optimization
\begin{equation}
  \label{eq:regnat}
  \min_{f\in\Fspace} \EE \loss(f(X), Y) \text{ s.t. }  f\in \InvF(\Reg)
\end{equation}

\begin{as}
$\Reg$ is such that   $\InvF(\Reg) \subset \InvF$
  \end{as}

The following corollary shows that minimizing the natural loss with constraint
is equivalent to solving the adversarial loss~\eqref{eq:advmin}
\begin{cor}
  \label{cor:constr}
  Any solution of the optimization program~\eqref{eq:regnat} with $\Reg$ satisfying (A1) is a minimizer of the adversarial loss.
\end{cor}
\begin{proof}
  Let us first write \fycomment{careful notation, $\PopLoss{\adv}$ currently equal $\PopLossReg{\adv}(\Reg)$}
  \begin{align*}
  \PopLoss{\adv}(f) &= \PopLoss{}(f) + [\PopLoss{\adv}(f) - \PopLoss{}(f)] \\
  &=  \EE \loss(\func_\param(\Trafo{X}{\Pert'}),\YID) +  \underbrace{\EE [\max_{\Pert' \in \Pertset} \loss(\func(\Trafo{X}{\Pert'}),\YID) - \loss(\func(X),\YID)]}_{\regadvnat(f)}
  \end{align*}
  By Theorem~\ref{theo:1} we know that $\frob \in \InvF$ minimizes $\PopLoss{\adv}(f)$. Hence, $\regadvnat(\frob) = 0$. This shows that the two optimization programs~\eqref{eq:advmin} and~\eqref{eq:regnat} are in fact equivalent.
\end{proof}
Note that both of these hold without assumption, i.e. even if $Y|X$ changes (but of course there will be a tradeoff, refer to tradeoff section).

\subsection{General penalized regularization framework}

Since minimizing in the set of feasible functions $f\in \InvF$ in the context of neural networks could be hard accomplish (i.e. simultaneously minimizing and feasibility could be hard), 
common practice is to relax the constraints by only requiring $f\in \InvF_\eps$, where we define
\begin{equation*}
  \InvF_{\eps} = \{f: \Reg(f) \leq \eps \quad \forall z\}
\end{equation*}
Consequently, instead of constrained optimization we can also use penalization on the natural loss by Lagrangian duality, and rewrite~\eqref{eq:regnat} as
\begin{equation}
  \label{eq:natpen}
  \PopLossReg{nat}(\Reg, \lambda) := \min_{f\in\Fspace} \EE_{X,Y} \loss(f(X),Y) + \lambda\Reg(f, X, X', Y)
\end{equation}

%% For $\eps=0$ many of them result in $\regadvnat(f) = 0$ in the Corollary (see Lemma~\ref{lem:regzero}).


In this paper we only consider regularizers $\Reg$ that satisfy $f\in \InvF \implies
\Reg(f) = 0$ (but not necessarily vice versa, i.e. TRADES). By Theorem~\ref{cor:constr} all robust
solutions $\frob \in\InvF$, and hence adding any of the above constraints
$\Reg_i(f,X) = 0$ to the robust loss would not change the minimizer of
the optimization problem since they are consequences of
$f\in\InvF$. Applying the same relaxation as above, yields penalized
adversarial training as follows
\begin{equation}
  \label{eq:advpen}
  \PopLossReg{rob}(\Reg, \lambda) := \min_{f\in\Fspace} \EE_{X,Y} \sup_{x'\in\SubGorbit{X}}\loss(f(x'),Y) + \lambda\Reg(f, X, X', Y)
\end{equation}
Compared to penalizing the natural loss, this optimization would
require searching two kind of adversarial examples: one that maximizes
$\loss(f(x'),Y)$ and one that solves the inner maximization in
the regularizer. ?? The regularizers which make sense in this setting are L2, TRADES, 

\paragraph{choosing two adversarial examples}

%% The next lemma shows that under the following assumption, the
%% adversarial examples are similar for two $h$. Where $f_i(x) = [f(x)]_i$.
%% \begin{as}
%%   \label{as:allequal}
%%   For $\regfunc$ that can be expressed as $\regfun(x,x') = \sum_{j=1}^d g(f_i(x), f_i(x'))$ we have for the cross-entropy loss $c' g(f_i(x_,f_i(x')) \leq  \log f_i(x') - \log f_i(x)$ 
%% \end{as}

%% \begin{lem}
%% Under Assumption~\ref{as:allequal} we have $\EE R(f, X, X', Y) \leq 
%% \end{lem}
We may run the modified regularized adversarial training instead to save on computation time:
\begin{equation}
  \label{eq:advpen}
  \PopLossReg{rob}(\regfunc, \lambda) := \min_{f\in\Fspace} \EE_{X,Y} \sup_{x'\in\SubGorbit{X}}\loss(f(x'),Y) + \lambda\Reg'(f, X, X^\star, Y)
\end{equation}
where now $\Reg'(f,X, X^\star, Y) = \regfunc(X, X^\star, Y)$, where $X^\star =  \arg\sup_{x'\in\SubGorbit{X}}\loss(f(x'),Y)$.
That makes ALP adv $= \PopLossReg{\rob}(h,\lambda)$.
\fycomment{maybe show some relation between $\PopLossReg{rob}(\Reg)$ vs. $\PopLossReg{rob}(\regfunc)$ under that assumption. It's an approximation }

We show in the appendix that empirically, it is best to choose
adversarial sample wrt. regularizer/loss and that it is as good as
choosing two adv. ex. 
\fycomment{to be seen}

%% Note that in this setting,
%% \begin{itemize}
%% \item  $\Reg(f,X, Y) =
%%   \|f(x')-f(X)\|_2^2$ with $x' = \argmax_{u\in\Gorbit{X}} \loss(f(u),Y)$ (ALP adv.) 
%% \end{itemize}

\fycomment{Does Regul. on adv. loss generally do worse/better?}
\fycomment{Trades claims that the key is that they don't enforce $\ell(f(x'),Y)$
to be small. How does TRADES with adv. loss compare with natural loss?}
%% \fycomment{we could make a point out of that $\Reg_4$, i.e. RECOVARIT
%%   does not need two kinds of adversarial examples. now that'd be
%%   interesting to compare against ~\eqref{eq:natpen} with $\Reg(f)$
%%   Trades in this view really seems the least founded (still don't get
%%   their proof but also general idea/logic seems much more handwavy/arbitrary
%%   than they make it seem)}


\subsection{Different choices of regularizers}
\label{sec:diffreg}

In this section we want to discuss the different regularizers $\Reg(f)$
that we want to compare, most of them already empirically explored
in the $\ell_\infty$ literature.
In general, they can all be united under one hood and expressed as
$\Reg_i(f,X,X',Y) = \sup_{x'\in\SubGorbit{X}} \regfunc_i(X, X', Y)$ for some $\regfunc$.
\begin{itemize}
\item $\regfunc_0(X,X',Y) =  \|f(X)-f(x')\|^2_2$ (L2, directly follows from theory)
\item $\regfunc_1(X, X', Y) = \loss(f(x'), f(X))$ (TRADES)
\end{itemize}
%% \begin{itemize}
%% \item $\Reg_0(f,X) =  \sup_{x'\in\SubGorbit{X}}\|f(x)-f(x')\|^2_2$ (L2)
%% \item $\Reg_1(f, X) = \sup_{x'\in\SubGorbit{X}}\loss(f(x'), f(X))$ (TRADES)
%% \end{itemize}
There is also non-adversarial $\Reg_4(f, X) = \EE_{x'\in\SubGorbit{X}}
\|f(x') -f(X)\|_2^2$ (CORE, not quite,) which is random augmentation -
but is not as effective \fycomment{have we tried?}

Note that regular adversarial training corresponds to $\lambda = 1$ and the following $\Reg(f)$.
The following ``regularizers'' require finding adversarial examples using the data label
\begin{itemize}
  \item $\Reg_2(f, X, Y) = \|f(x')-f(X)\|_2^2$ with $x' = \argmax_{u\in\Gorbit{X}} \loss(f(u),Y)$ (ALP plain)
  \item $\regfunc_3(f, X, X', Y) = \loss(f(x'),Y) - \loss(f(X),Y)$
(ordinary adv. Training with adv. batch with $\lambda=1$)
\item $\regfunc_4(f, X, X',Y) = \loss(f(x'),Y)$ (ordinary
  Adv. Training mixed batc h ($\lambda=1$)).
  \item $\regfunc_5(f, X, X', Y) = |\loss(f(x'),Y) - \loss(f(X),Y)|$ (modified adv. training) \fycomment{only diff is that it not always tries to find misclassified samples like Ord. ART, but actual ones with different loss (closer to regularization on function}
\end{itemize}
In fact all adversarial examples here are the same (maximizer of cross entropy loss for fixed $Y$).

Note that for $i=0, 3, 4$ that $\InvF(\Reg_i) \subset \InvF$ and
hence the solution of the corresponding constrained
problem~\eqref{eq:regnat} is a minimizer of the adversarial loss
\fycomment{under which loss conditions can you show the same for trades? otherwise say
how it approximates}

\paragraph{Comparing different regularizers}
%% Some guesses how the different $h_i$ are related - or maybe even experiments
%% about how big the difference of $h_j(x_j) - h_i(x_j) $ are on real data
%% or just some experiment in our framework

Each of the regularizers suggests choosing different adversarial examples.
These two groups are conceptually different: One that is trying
to match predictions for different $x$ within $\SubGorbit{x}$ and
another that depends on $Y$ and is matching the losses. I.e. if the
loss is currently big on $X$, find $X'$ that has small loss and if loss on $X'$ small,
find big loss/misclassified $X'$.

For fixed $\lambda$, we have $\PopLoss{nat}(\Reg_1) \geq \PopLoss{nat}(\Reg_0)$.
hence it is more restrictive to 


I'm guessing adversarial example wrt. CE or Reg. doesn't make a huge difference.
The reason is that they are closely related. In particular with unsigned ones
it depends on the loss satisfying regularity conditions
\fycomment{we can run experiment to verify this here} This entails
that the key is the actual regularizer, not necessarily the
regularizer we use to find $f$. In simulations we see that (at least for
wo-10, for FO, obviously they're going to wonder off in
$\ell_2$-distance), it picks similar sample -> can just choose the one
for CE.

\paragraph{Comparing $\PopLoss{adv}$ vs. $\PopLoss{nat}$ (falsifying TRADES ``explanation''?)}
There is a categorical difference between $x$ related regularizers and
$x, y$ related ones.  the $X$ ones are focusing on functional
``smoothness'' no matter where on or off the boundary.

Although all regularizers serve to make the predictions between adversarial
and regular example closer, 
it is hard to predict which regularizer would lead to the best practical
results for deep neural networks, but at least by Theorem 1, every minimizer of
the robust loss should be in the sets $\InvF_{\eps}(\Reg)$ for all of the regularizers above
and all $\eps \geq 0$ and vice versa. 

TRADES argue that whether one or the other prevails is somewhat dependent on
regularization.

\fycomment{Does the actual example or regularizer make the difference?? it should
be the regularizer itself}
\begin{itemize}
\item It is interesting to directly compare ALP plain against L2 
i.e. same regularizer for backprop but different adversarial example

\item Similarly interesting to compare TRADES with usual adv. training but
with different $\lambda$. Is it their tuning that made the difference
or combo of (1) adv. sample search wrt $Y$ and (2) asymmetric loss
\end{itemize}

My guess: sometimes these examples probably match (more so for wo-10 than FO)
in other cases when you use the wrong sample ($Y$ dependent) for the ``right''
regularizer, it is just not as strong for the regularizer


\subsection{Trade-off between nat. and robust accuracy}

\fycomment{put into perspective with TRADES}

Note that in natural applications such as classification, the goal to
obtain robustness is only meaningful when the conditional distribution
of $Y$ does not change too much with a transformation, that is
When $Y|X$ is the same within an orbit (and hence suborbit), or more formally
\begin{equation}
  \label{eq:robustsense}
  P(Y|\{X = x\}) = p_z \quad \forall x\in\SubGorbit{z}, z.
\end{equation}
When this assumption holds, we show in this section that there is no trade-off
between natural and robust accuracy.

First of all, we want to discuss the sensibility of property~\eqref{eq:robustsense}.
If this assumption does not hold for the combination of (transformation, distribution), then being
able to assign the same predicted value $Y$ to both $X$ and
$\Trafo{X}{\Pert}$ under arbitrary transformations $\Pert in \Pertset$
is not interpretable nor meaningful. Why would it be desirable to have a model
which predicts a value for a transformation that has zero probability to occur in
the actual distribution?

Let us illustrate the sensibility of this assumption for image classification: Say we have two
features = (texture, shape). In the true distribution, elephant always
comes with this greyish skin texture and cat with
theirs. P(cat texture, elephant shape)=0. Now we can learn a
classifier that is "robust" against texture changes and only focuses
on shape. But what does it mean to classify (cat texture,
elephant shape) as elephant? I have a hard time understanding the
relevance of this. Now the texture work is interesting in its own
right, understand what imagenet features learn. But the robustness
question asked in this setting would be questionable in terms of
sensibility.

We now formally state the theorem that shows that under this
reasonable assumption there is no trade-off
\begin{theo}
  Under assumption~\eqref{eq:robustsense}, if
  $\InvF \subset \Fspace$ and the loss is continuous in the first
  argument, then there exists $\fbest \in \InvF$ such that
  $\PopLoss{}(\fbest) \leq \PopLoss{}(f)$ for all
  $f\in \Fspace$.   
\end{theo}

\begin{proof}
  \fycomment{Notationally not perfectly rigorous, but to illustrate the point}
  We prove existence by construction: Take any minimizer $\fhat$ of $\PopLoss{}(f)$ which is not in  $\InvF$.
  We can then construct an $\fbest$, such that $ \PopLoss{\adv}(\fbest) = \PopLoss{\nat}(\fbest) = \PopLoss{\nat}(\fhat)$.
  The construction is as follows: First note that because of measurability of $\EE_Y [\loss(f(X), Y) | X ]$ ``wrt. $f(X)$'' conditioned on $\Gorbit{x}$ we have for any function $f$ that
  \begin{align*}
    \EE_{\Gorbit{x}} \EE_X [\EE_Y [\loss(f(X), Y) | X ] | \Gorbit{x}] &=  \EE_{\Gorbit{x}} \EE_X [ \EE_Y [\loss(f(X), Y) | f(X)] \Gorbit{x}]
  \end{align*}
  Given a fixed $\Gorbit{x}$, let us now define $\fbest$ on all $x' \in \Gorbit{x}$ as a constant, i.e. $\fbest(x') = c(\Gorbit{x})$ which satisfies:
  $\EE_Y \loss(c(\Gorbit{x}), Y)| \Gorbit{x} = \EE_{X,Y} \loss(\fhat(X), Y)| \Gorbit{x}$. Since we assume that $\loss$ is continuous, by Rolle's theorem
  such a $c(\Gorbit{x})$ exists. Now $\fbest \in \InvF$ and since $\InvF \in \Fspace$ we have
  \begin{align*}
    \PopLoss{}(\fbest) = \EE \loss(\fbest(X), Y)  &=  \EE_{\Gorbit{x}} \EE_X [ \EE_Y [\loss(\fbest(X), Y) | \fbest(X)] \Gorbit{x}] \\
    &= \EE_{\Gorbit{x}} \EE_{X,Y} [\loss(\fhat(X), Y) | \Gorbit{x} ] = \PopLoss{}(\fhat).
  \end{align*}
  Since  $\fhat$ is a minimizer of the population loss, we also have $\PopLoss{}(\fbest) \leq \PopLoss{}(f)$ for all $f\in\Fspace$ q.e.d. 
\end{proof}

This requirement is realistic in a practical data
generation setting described in the next section.



\paragraph{Example distribution}
\fycomment{have to carefully think whether notation is necessary}
The condition~\ref{eq:robustsense} is fulfilled for any model where $Y \ortho X \big| \XID{\ID}$, since we then have
\begin{align*}
Y|\{X=x\}, \XID{\ID} \overset{d}{=} Y|\XID{\ID} \implies Y | \{X=x\} \overset{d}{=} Y | \XID{\ID}(x) \quad \forall x.
\end{align*}
An explicit example generative model that simulates the natural process
of image capturing is depicted in a probabilistic model like in Figure ~\ref{fig:dag}.

\fycomment{have to unify notation}
Let us go through the model in detail. Randomness comes from $\ID$ and $\Pert$. We have a group $\Group$ of transformations $\Trafo{\cdot}{\Pert}$
of $\X$ onto itself. 
We denote by $\XID{\ID}$ the $\Group$-orbit of $x$, that is
\begin{equation*}
\XID{\ID} \defn \{ \Trafo{x}{\Pert}: \Trafo{\cdot}{\Pert} \in \Group\}  
\end{equation*}
The parameter $\Pert$ then picks one sample from $\XID{\ID}$ according to some distribution which becomes the random variable $X$. It is also assumed that there is a unique mapping $v : \X \to \allorbits$ from the domain $\X$ to the space of orbits $\allorbits$ (that is the orbits are disjoint subsets in $\X$).
Now note that in this model,
we have that $X, \Trafo{X}{\Pert'}$ follow the same distribution for any perturbation $\Pert'$ and furthermore because of conditional independence 


\fycomment{The $\Pert$ in the graphical model should now be $\SubGorbit{X}$, else it's confusing, generally figure needs revamp}

\begin{figure}[htbp]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=.6\columnwidth]{images/PP_DAG4.pdf}}
%\vspace{-.1in}
\caption{\small Generative model for observations $\ID, X, Y$. %Source of randomness are $\ID, \Pert$.
Here, the sources of randomness are the
perturbation $\Pert$ and the $\ID$.
%with a latent random perturbation $\Pert$.
The generative probabilistic model is rooted in the intuition that the
process of collecting an observation always starts with randomly
picking an object with a certain $\ID$ with associated attributes
$\attvec = [\attstyle,\attcore]$ (usually unobserved) which determine
its identity uniquely. The class $\YID$ is a deterministic function of
the core attributes $\attcore$ and $\XID{\ID} \in \RN^d$ is an
arbitrary function of $\attvec$ and assumed to be deterministic as
well.  The observed image $X \in \RN^d$ %added to the dataset is a
random transformation, defined by a perturbation $\Pert \in \Pertset
\subset \RN^\dimpert$, of $\XID{\ID}$, i.e.\ $X =
\Trafo{\XID{\ID}}{\Pert}$. For instance for images, the transformation
$\Trafo{\cdot}{\Pert}$ with perturbation $\Pert$ could consist of a
rotation with degree $\Pert \in [-30^{\circ},30^{\circ}]$, which arises
naturally from the image capturing process.
$\ID$ is a unique identifier variable encoding the identity of the underlying object. $\Trafo{\XID{\ID}}{\Pert}$ with perturbation $\Pert$ describes the transformation of $\XID{\ID}$ arising in the measurement process recording $X$.}
\label{fig:dag}
\end{center}
\vskip -0.2in
\end{figure}




\section{Spatial-equivariant networks}

\subsection{Two-Stage predictor}



==> main_results.tex <==
\begin{table*}[ht]
\caption{Natural and grid accuracies of different models}
\vskip 0.15in
\begin{center}
  \begin{tabular}{c  c  c  c c}
    \hline
    

\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
&  $\recovarit{\atabb}{\woabb{10}}{50}$
    & {93.44\% (0.19\%)} & 68.14\% (0.48\%) \\
&  $\recovarit{\atabb}{\woabb{10}}{100}$
    & 92.05\% (0.25\%) & 70.35\% (0.17\%) \\
& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1$)
    & 91.13\% (0.13\%) & {\bf 75.89\% (0.23\%)}  \\
 \cdashline{2-4}
%%%%% FO %%%%%%%%%%
& $\recovarit{\atabb}{\fo}{50}$ 
	& 92.19\% (0.23\%) & 64.26\% (0.25\%)\\
& $\recovarit{\atabb}{\fo}{100}$ 
	& 91.83\% (0.19\%)& 69.74\% (0.27\%)\\
& $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 3$)
	& 89.70\% (0.10\%) & {\bf 77.72\% (0.35\%)}\\

\hline                                                                              
\multirow{6}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
%& Standard
%    & 70.23\% (0.18\%) & 5.09\% (0.25\%)  \\
%%& No Crop
%%    & 66.42\% (0.30\%) & 0.86\% (0.08\%)  \\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%	
%&  $\recovarit{\atabb}{\woabb{1}}{50}$
%	& 72.38\% (0.17\%) & 23.43\% (0.47\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 66.62\% (0.37\%) & 28.53\% (0.25\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 0.75$)
%	& 66.54\% (0.26\%) & {\bf 45.97\% (0.22\%)}\\
%	\cdashline{2-4}
%%%%% Worst-of-10 %%%%%%%%%%
&  $\recovarit{\atabb}{\woabb{10}}{50}$
    & {73.03\% (0.13\%)} & 35.93\% (0.24\%) \\
&  $\recovarit{\atabb}{\woabb{10}}{100}$
    & 68.79\% (0.34\%) & 38.21\% (0.10\%) \\
& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 0.25$)
    & 68.54\% (0.27\%) & {\bf 49.30\% (0.33\%)} \\
\cdashline{2-4}
%%%%% FO %%%%%%%%%%
& $\recovarit{\atabb}{\fo}{50}$ 
	& 71.11\% (0.37\%) & 33.40\% (0.21\%) \\
& $\recovarit{\atabb}{\fo}{100}$ 
	& 68.87\% (0.19\%) & 37.87\% (0.12\%) \\
&$\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 0.5$)
	&  68.44\% (0.39\%) & {\bf 52.58\% (0.20\%)} \\

\end{tabular}}
\end{center}
\end{table*}


==> reg_table.tex <==
\begin{table*}[ht]
  \begin{center}
    \caption{blabla\label{tab:reg}}
      %{\stdaug refers to data augmentation, i.e. \ltwo (\advb, \dataug, \rnd). Accuracies of different models trained with $\woabb{1}$ defenses (corresponding to data augmentation) and evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on the CIFAR-10 and CIFAR-100 datasets.
\vskip 0.15in
\begin{tabular}{c c c c c c c c}
  & \std & \stdaug
  & A.T. & \stdaug (\ltwo) & \makecell{\ltwo \\(\natb, \advreg, \woabb{10})}
  & \makecell{\trades \\ (\natb, \advreg, \woabb{10})} & \makecell{\ALP\\(\mixb, \advreg, \fo)} \\
  \hline
  SVHN (nat) & 00.00\% & 00.00\% & 00.00\% & 99.99\% & 90.73\% & 00.00\% & 0.00\% \\
  \qquad\: (grid) & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
  \hline
  CIFAR (nat) & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
  \qquad\quad (grid) & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
  \hline
\end{tabular}
\end{center}
\end{table*}
  


%% \begin{center}
%% {\renewcommand{\arraystretch}{1.4}
%% \begin{tabular}{cl|ccc|cc|cc}
%% & \diagbox{Training}{Evaluation} & Natural & Grid  \\

%%  \hline
%%  \multirow{4}{*}{\rotatebox[origin=c]{90}{SVHN}}
%%  %%%%% Standard %%%%%%%%%%
%%  & Standard
%%      & 95.48\% (0.15\%) & 18.85\% (1.27\%)\\
%%  \cdashline{2-4}
%%  %%%%% Worst-of-1 %%%%%%%%%%	
%%  &  $\recovarit{\atabb}{\woabb{1}}{50}$
%%  	& 96.19\% (0.06\%) & 80.43\% (0.14\%)\\
%%  &  $\recovarit{\atabb}{\woabb{1}}{100}$
%%  	& 93.97\% (0.09\%) & 82.60\% (0.23\%)\\
%%  & $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%%  	& 96.19\% (0.07\%) & {\bf 90.48\% (0.15\%)}\\ 
%% \hline
%% \multirow{4}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
%% %%%%% Standard %%%%%%%%%%
%% & Standard
%%     & 92.11\% (0.18\%) & 9.52\% (0.66\%)  \\
%% %& No Crop
%% %    & 90.50\% (0.22\%) & 1.63\% (0.21\%)  \\
%% \cdashline{2-4}
%% %%%%% Worst-of-1 %%%%%%%%%%
%% &  $\recovarit{\atabb}{\woabb{1}}{50}$
%% 	& 92.96\% (0.17\%) & 51.27\% (0.45\%)\\
%% &  $\recovarit{\atabb}{\woabb{1}}{100}$
%% 	& 89.93\% (0.18\%) & 58.29\% (0.60\%)\\
%% & $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%% 	& 89.43\% (0.28\%) & {\bf 71.97\% (0.11\%)}\\
%% 	\cdashline{2-4}
%% \hline                                                                              
%% \multirow{4}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
%% & Standard
%%     & 70.23\% (0.18\%) & 5.09\% (0.25\%)  \\
%% %& No Crop
%% %    & 66.42\% (0.30\%) & 0.86\% (0.08\%)  \\
%% \cdashline{2-4}
%% %%%%% Worst-of-1 %%%%%%%%%%	
%% &  $\recovarit{\atabb}{\woabb{1}}{50}$
%% 	& 72.38\% (0.17\%) & 23.43\% (0.47\%)\\
%% &  $\recovarit{\atabb}{\woabb{1}}{100}$
%% 	& 66.62\% (0.37\%) & 28.53\% (0.25\%)\\
%% & $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 0.75$)
%% 	& 66.54\% (0.26\%) & {\bf 45.97\% (0.22\%)}\\
%% 	\cdashline{2-4}
%% \end{tabular}}
%% \end{center}
%% \end{table*}


==> svhn_table.tex <==
\begin{table*}[htp]
  \caption{Mean accuracies of different models trained with and without defenses and evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on the SVHN dataset. Standard errors are shown in parentheses.}
    \label{tab:wok_svhn}
\vskip 0.15in

\begin{center}
{\renewcommand{\arraystretch}{1.4}
\begin{tabular}{cl|ccc|cc|cc}
& \diagbox{Training}{Evaluation} & Natural & Grid  \\
\hline
\multirow{13}{*}{\rotatebox[origin=c]{90}{SVHN}}
%%%%%% Standard %%%%%%%%%%
& Standard
    & 95.48\% (0.15\%) & 18.85\% (1.27\%)\\
\cdashline{2-4}
%%%%% Worst-of-1 %%%%%%%%%%	
&  $\recovarit{\atabb}{\woabb{1}}{50}$
	& 96.19\% (0.06\%) & 80.43\% (0.14\%)\\
&  $\recovarit{\atabb}{\woabb{1}}{100}$
	& 93.97\% (0.09\%) & 82.60\% (0.23\%)\\
& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
	& 96.19\% (0.07\%) & {\bf 90.48\% (0.15\%)}\\ 
\cdashline{2-4}
%%%%% Worst-of-10 %%%%%%%%%%		
&  $\recovarit{\atabb}{\woabb{10}}{50}$
    & {96.56\% (0.07\%)} & 88.83\% (0.10\%) \\
&  $\recovarit{\atabb}{\woabb{10}}{100}$
    & 95.92\% (0.03\%) & 89.75\% (0.17\%) \\
& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1.5$)
    & 96.41\% (0.07\%) & {\bf 92.17\% (0.11\%)}  \\
\cdashline{2-4}
%%%%% Worst-of-20 %%%%%%%%%%		
&  $\recovarit{\atabb}{\woabb{20}}{50}$
    & 96.60\% (0.06\%) & 89.72\% (0.17\%) \\
&  $\recovarit{\atabb}{\woabb{20}}{100}$
    & 96.29\% (0.14\%) & 90.57\% (0.20\%) \\
& $\recovarit{\acronymmath}{\woabb{20}}{50}$ ($\lambda = 1.5$)
    & 96.39\% (0.04\%) & {\bf 92.48\% (0.05\%)} \\
\cdashline{2-4}
%%%%% FO %%%%%%%%%%
& $\recovarit{\atabb}{\fo}{50}$ 
	& 96.27\% (0.00\%) &  84.81\% (0.01\%)\\
& $\recovarit{\atabb}{\fo}{100}$ 
	& 96.06\% (0.10\%) & 87.29\% (0.09\%)\\
& $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 2.5$)
	& 96.30\% (0.09\%) & {\bf 92.42\% (0.20\%)}\\    
%\hline
%\multirow{13}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
%%%%%% Standard %%%%%%%%%%
%& Standard
%    & 92.11\% (0.18\%) & 9.52\% (0.66\%)  \\
%%& No Crop
%%    & 90.50\% (0.22\%) & 1.63\% (0.21\%)  \\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%
%&  $\recovarit{\atabb}{\woabb{1}}{50}$
%	& 92.96\% (0.17\%) & 51.27\% (0.45\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 89.93\% (0.18\%) & 58.29\% (0.60\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
%	& 89.43\% (0.28\%) & {\bf 71.97\% (0.11\%)}\\
%\cdashline{2-4}
%%%%%% Worst-of-10 %%%%%%%%%%
%&  $\recovarit{\atabb}{\woabb{10}}{50}$
%    & {93.44\% (0.19\%)} & 68.14\% (0.48\%) \\
%&  $\recovarit{\atabb}{\woabb{10}}{100}$
%    & 92.05\% (0.25\%) & 70.35\% (0.17\%) \\
%& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 1$)
%    & 91.13\% (0.13\%) & {\bf 75.89\% (0.23\%)}  \\
% \cdashline{2-4}
%%%%%% Worst-of-20 %%%%%%%%%%		
%&  $\recovarit{\atabb}{\woabb{20}}{50}$
%    & 93.46\% (0.17\%) & 69.98\% (0.22\%) \\
%&  $\recovarit{\atabb}{\woabb{20}}{100}$
%    & 92.15\% (0.28\%) & 72.31\% (0.20\%) \\
%& $\recovarit{\acronymmath}{\woabb{20}}{50}$ ($\lambda = 1$)
%    & 90.67\% (0.12\%) & {\bf 76.72\% (0.21\%)} \\
%    \cdashline{2-4}
%%%%%% FO %%%%%%%%%%
%& $\recovarit{\atabb}{\fo}{50}$ 
%	& 92.19\% (0.23\%) & 64.26\% (0.25\%)\\
%& $\recovarit{\atabb}{\fo}{100}$ 
%	& 91.83\% (0.19\%)& 69.74\% (0.27\%)\\
%& $\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 3$)
%	& 89.70\% (0.10\%) & {\bf 77.72\% (0.35\%)}\\
%\hline                                                                              
%\multirow{13}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
%%%%%% Standard %%%%%%%%%%
%& Standard
%    & 70.23\% (0.18\%) & 5.09\% (0.25\%)  \\
%%& No Crop
%%    & 66.42\% (0.30\%) & 0.86\% (0.08\%)  \\
%\cdashline{2-4}
%%%%%% Worst-of-1 %%%%%%%%%%	
%&  $\recovarit{\atabb}{\woabb{1}}{50}$
%	& 72.38\% (0.17\%) & 23.43\% (0.47\%)\\
%&  $\recovarit{\atabb}{\woabb{1}}{100}$
%	& 66.62\% (0.37\%) & 28.53\% (0.25\%)\\
%& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 0.75$)
%	& 66.54\% (0.26\%) & {\bf 45.97\% (0.22\%)}\\
%	\cdashline{2-4}
%%%%%% Worst-of-10 %%%%%%%%%%
%&  $\recovarit{\atabb}{\woabb{10}}{50}$
%    & {73.03\% (0.13\%)} & 35.93\% (0.24\%) \\
%&  $\recovarit{\atabb}{\woabb{10}}{100}$
%    & 68.79\% (0.34\%) & 38.21\% (0.10\%) \\
%& $\recovarit{\acronymmath}{\woabb{10}}{50}$ ($\lambda = 0.25$)
%    & 68.54\% (0.27\%) & {\bf 49.30\% (0.33\%)} \\
%\cdashline{2-4}
%
%%%%%% Worst-of-20 %%%%%%%%%%		
%&  $\recovarit{\atabb}{\woabb{20}}{50}$
%    & 73.33\% (0.22\%) & 38.06\% (0.19\%) \\
%&  $\recovarit{\atabb}{\woabb{20}}{100}$
%    & 69.15\% (0.49\%) & 40.09\% (0.31\%) \\
%& $\recovarit{\acronymmath}{\woabb{20}}{50}$ ($\lambda = 0.25$)
%    & 68.04\% (0.27\%) & {\bf 49.98\% (0.31\%)} \\
%    \cdashline{2-4}
%%%%%% FO %%%%%%%%%%
%& $\recovarit{\atabb}{\fo}{50}$ 
%	& 71.11\% (0.37\%) & 33.40\% (0.21\%) \\
%& $\recovarit{\atabb}{\fo}{100}$ 
%	& 68.87\% (0.19\%) & 37.87\% (0.12\%) \\
%&$\recovarit{\acronymmath}{\fo}{50}$ ($\lambda = 0.5$)
%	&  68.44\% (0.39\%) & {\bf 52.58\% (0.20\%)} \\
\end{tabular}}
\end{center}
\end{table*}



==> wo1_table.tex <==
\begin{table*}[ht]
\caption{Accuracies of different models trained with $\woabb{1}$ defenses (corresponding to data augmentation) and evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on the CIFAR-10 and CIFAR-100 datasets. \label{tab:wo1_main}}
\vskip 0.15in
\begin{center}
{\renewcommand{\arraystretch}{1.4}
\begin{tabular}{cl|ccc|cc|cc}
& \diagbox{Training}{Evaluation} & Natural & Grid  \\

 \hline
 \multirow{4}{*}{\rotatebox[origin=c]{90}{SVHN}}
 %%%%% Standard %%%%%%%%%%
 & Standard
     & 95.48\% (0.15\%) & 18.85\% (1.27\%)\\
 \cdashline{2-4}
 %%%%% Worst-of-1 %%%%%%%%%%	
 &  $\recovarit{\atabb}{\woabb{1}}{50}$
 	& 96.19\% (0.06\%) & 80.43\% (0.14\%)\\
 &  $\recovarit{\atabb}{\woabb{1}}{100}$
 	& 93.97\% (0.09\%) & 82.60\% (0.23\%)\\
 & $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
 	& 96.19\% (0.07\%) & {\bf 90.48\% (0.15\%)}\\ 
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
%%%%% Standard %%%%%%%%%%
& Standard
    & 92.11\% (0.18\%) & 9.52\% (0.66\%)  \\
%& No Crop
%    & 90.50\% (0.22\%) & 1.63\% (0.21\%)  \\
\cdashline{2-4}
%%%%% Worst-of-1 %%%%%%%%%%
&  $\recovarit{\atabb}{\woabb{1}}{50}$
	& 92.96\% (0.17\%) & 51.27\% (0.45\%)\\
&  $\recovarit{\atabb}{\woabb{1}}{100}$
	& 89.93\% (0.18\%) & 58.29\% (0.60\%)\\
& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 3.5$)
	& 89.43\% (0.28\%) & {\bf 71.97\% (0.11\%)}\\
	\cdashline{2-4}
\hline                                                                              
\multirow{4}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
& Standard
    & 70.23\% (0.18\%) & 5.09\% (0.25\%)  \\
%& No Crop
%    & 66.42\% (0.30\%) & 0.86\% (0.08\%)  \\
\cdashline{2-4}
%%%%% Worst-of-1 %%%%%%%%%%	
&  $\recovarit{\atabb}{\woabb{1}}{50}$
	& 72.38\% (0.17\%) & 23.43\% (0.47\%)\\
&  $\recovarit{\atabb}{\woabb{1}}{100}$
	& 66.62\% (0.37\%) & 28.53\% (0.25\%)\\
& $\recovarit{\acronymmath}{\woabb{1}}{50}$ ($\lambda = 0.75$)
	& 66.54\% (0.26\%) & {\bf 45.97\% (0.22\%)}\\
	\cdashline{2-4}
\end{tabular}}
\end{center}
\end{table*}

==> wo1_table_narrow.tex <==
%\vskip -0.15in
\begin{table}[t]
\caption{\small Mean accuracies of different models trained with $\woabb{1}$ defenses (corresponding to data augmentation) and ``Standard'' training (cf.\ Section~\ref{sec:datasets}). The models are evaluated on the natural test set (column ``Natural'') and against the grid search attack (column ``Grid'') on the CIFAR-10 and CIFAR-100 datasets. \label{tab:wo1_main}}
\begin{center}
{\renewcommand{\arraystretch}{1.4}
\begin{tabular}{cl|ccc|cc|cc}
& \diagbox{Training}{Evaluation} & Natural & Grid  \\

 \hline
 \multirow{4}{*}{\rotatebox[origin=c]{90}{SVHN}}
 %%%%% Standard %%%%%%%%%%
 & Standard
     & 95.48\%  & 18.85\%\\
 \cdashline{2-4}
 %%%%% Worst-of-1 %%%%%%%%%%	
 &  $\recovarit{\atabb}{\woabb{1}}{50}$
 	& 96.19\%& 80.43\%\\
 &  $\recovarit{\atabb}{\woabb{1}}{100}$
 	& 93.97\%& 82.60\%\\
 & $\recovarit{\acronymmath}{\woabb{1}}{50}$
 	& 96.19\%& {\bf 90.48\%}\\ 
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{CIFAR-10}}
%%%%% Standard %%%%%%%%%%
& Standard
    & 92.11\% & 9.52\% \\
%& No Crop
%    & 90.50\% (0.22\%) & 1.63\% (0.21\%)  \\
\cdashline{2-4}
%%%%% Worst-of-1 %%%%%%%%%%
&  $\recovarit{\atabb}{\woabb{1}}{50}$
	& 92.96\% & 51.27\%\\
&  $\recovarit{\atabb}{\woabb{1}}{100}$
	& 89.93\% & 58.29\% \\
& $\recovarit{\acronymmath}{\woabb{1}}{50}$
	& 89.43\% & {\bf 71.97\% }\\
	\cdashline{2-4}
\hline                                                                              
\multirow{4}{*}{\rotatebox[origin=c]{90}{CIFAR-100}}
& Standard
    & 70.23\% & 5.09\% \\
%& No Crop
%    & 66.42\% (0.30\%) & 0.86\% (0.08\%)  \\
\cdashline{2-4}
%%%%% Worst-of-1 %%%%%%%%%%	
&  $\recovarit{\atabb}{\woabb{1}}{50}$
	& 72.38\%& 23.43\%\\
&  $\recovarit{\atabb}{\woabb{1}}{100}$
	& 66.62\%& 28.53\%\\
& $\recovarit{\acronymmath}{\woabb{1}}{50}$
	& 66.54\%& {\bf 45.97\%}\\
\end{tabular}}
\end{center}
\end{table}
%\vskip -0.1in
